Tree-Structured Modelling of Categorical Predictors in Regression

Generalized linear and additive models are very efficient regression tools but the selection of relevant terms becomes difficult if higher order interactions are needed. In contrast, tree-based methods also known as recursive partitioning are explicitly designed to model a specific form of interaction but with their focus on interaction tend to neglect the main effects. The method proposed here focusses on the main effects of categorical predictors by using tree type methods to obtain clusters. In particular when the predictor has many categories one wants to know which of the categories have to be distinguished with respect to their effect on the response. The tree-structured approach allows to detect clusters of categories that share the same effect while letting other variables, in particular metric variables, have a linear or additive effect on the response. An algorithm for the fitting is proposed and various stopping criteria are evaluated. The preferred stopping criterion is based on $p$-values representing a conditional inference procedure. In addition, stability of clusters are investigated and the relevance of variables is investigated by bootstrap methods. Several applications show the usefulness of tree-structured clustering and a small simulation study demonstrates that the fitting procedure works well.

==> Simulation.tex <==
\section{Simulations }





One of the most important questions when building a tree is the choice of a optimal stopping criterion. In our applications we used a stopping criterion based on $p$-values of the likelihood-ratio statistic. To investigate the performance of the structured tree, especially the ability to form correct clusters, and to compare  stopping criteria, we now give the results of a small simulation study.

\begin{figure}[!ht]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_MSEordinal}&\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_MSEnominal}
\end{tabular}
\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_MSElinear}
\caption{Mean squared errors (MSEs) of parameter estimates of ordinal, nominal predictors and the linear term for the simulation study.}
\label{fig:BigSim_MSE}
\end{figure}


We consider the case of 4 ordinal and 4 nominal predictors in the tree component of our model. For both types of variables we use two predictors with 10 and two predictors with 5 categories. The true coefficients of the ordinal predictors are $(0,1,1,2,2,3,3,4,4)^\top$, $(0,0,0,0,2,2,2,2,2)^\top$, $(1,1,2,2)^\top$ and $(0,0,0,0)^\top$. For the nominal predictor they are $(0,0.5,0.5,-0.5,-0.5,1.5,1.5,-1.5,-1.5)^\top$, $(0,0,0,0,-2,-2,-2,-2,-2)^\top$, $(1,1,-1,-1)^\top$ and $(0,0,0,0)^\top$. In both cases the true numbers of clusters are 5, 2 and 3. The fourth predictor is not influential. Note that the effect of the first category in each case is set to zero. All in all there are 52 possible splits in the tree component. The true model contains 14 splits, 7 within the ordinal and 7 within the nominal predictors. We generate data sets with $n=2000$ observations and a normal distributed response with $\epsilon \sim N(0,1)$. Our model has an additional linear term $\xb^T\betab$, where $\xb$ is $N(\bf{0}_5,\Sigmab_5)$-distributed with variances 1 and covariances 0.3. The true regression coefficients of the linear term are $\betab=(-2,1,-1,3,2)^\top$.

The estimated coefficients are compared to the true parameters by calculating mean squared errors (MSEs). Therefore we distinguish between the tree-based parameters $\alphab$ and the parameters $\betab$ of the linear term. For  the $i$-th predictor  the MSE of the $\alpha$-parameters is $\sum_{j=1}^{m_i} (\hat{\alpha}_{ij}-\alpha_{ij})/(m_i)$ and for the $\beta$-parameters it is $\sum_{i=1}^{5} (\hat{\beta}_i-\beta_i)/5$.

In our analysis we distinguish between the MSE for the nominal and the MSE for the ordinal predictors respectively as the average over the four predictors. Boxplots of the computed MSEs based on 100 simulations are shown in Figure \ref{fig:BigSim_MSE}. We compare six different stopping criterions: AIC, BIC, 5-fold cross validation, 10-fold cross validation, $p$-values with significance level $\alpha=0.05$ and $p$-values with $\alpha=0.1$.  In Figure \ref{fig:BigSim_MSE} the latter are denoted by $p(0.05)$ and $p(0.1)$. The smallest median of MSEs for the ordinal predictors as well as for the nominal predictors were found for the strategy with p-values and common significance level $\alpha=0.05$ (fifth boxplots). MSEs for the linear term are very small and almost indentical over stopping criteria. Estimation of the linear term of the structured tree shows very good performance and seems to be not strongly linked to the clustering in the tree component.



In addition to the MSEs the number of clusters found by the algorithm are of interest.
Therefore, Figure \ref{fig:BigSim_ncluster} shows the number of splits in the tree component of the model separately for the ordinal and the nominal predictors. The horizontal line shows the optimal number of splits of the underlying data generating model. It is seen that  for ordinal predictors one obtains nearly perfect results with BIC and $p$-value  $\alpha=0.05$. The true number of 7 splits is found in almost all simulations. For nominal predictors the  performance  is very similar over stopping criteria with the exception of AIC, which performs worse than the other procedures. Since  for $p$-values with $\alpha=0.05$ there is no outlier it shows again the best performance. In summary, the number of splits very close to the optimal number for all the procedures showing that the model is able to find the right number of splits.


\begin{figure}[!ht]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_nclusterordinal}&\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_nclusternominal}
\end{tabular}
\caption{Number of splits of ordinal and nominal predictors in the tree component of the structured tree for the simulation study.}
\label{fig:BigSim_ncluster}
\end{figure}

\begin{figure}[!ht]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_fpfnordinal}&\includegraphics[width=0.5\textwidth]{Graphiken/BigSim_fpfnnominal}
\end{tabular}
\caption{FPR (left boxplots) and FNR (right boxplots) of ordinal and nominal predictors in the tree component of the structured tree for the simulation study.}
\label{fig:BigSim_fpfn}
\end{figure}

To check if the algorithm does not only find the right number of splits but also the correct clusters, False Positive and False Negative Rates (FPR/FNR) are computed.

\begin{itemize}
\item False Positive: A difference between two estimated parameters $\hat{\alpha}_{ij}$ which is truly zero is set to nonzero
\item False Negative: A difference between two estimated parameters $\hat{\alpha}_{ij}$ which is truly nonzero is set to zero
\end{itemize}

Figure \ref{fig:BigSim_fpfn} shows boxplots of TPR and FPR seperatly for the ordinal and nominal predictors. As for MSEs we compute the average over the four predictors. Since the structured tree has a weak tendency to overestimate the number of splits (see Figure \ref{fig:BigSim_ncluster}) FNRs are found to be zero in all simulations. With exception of AIC also the median of the FPRs is zero over stopping criteria.

In summary, the simulation study shows that  structured trees are able to identify the number of clusters rather correctly and yield very low false positive and negative rates. The algorithm  reduces the model complexity of categorical explanatory variables in the presence of smooth components very precisely.


==> header.tex <==
%% neu 1.9.2011     Abstände zwischen den Einträgen des Literaturverzeichnisses variieren.



%% Schrift
%\usepackage{mathptmx}
%\usepackage[scaled=.90]{helvet}
%\usepackage{courier}



\usepackage{times}      % old but good
%\usepackage{lmodern} %Latex STandard Schrift


%% language, coding
\usepackage[german,english]{babel}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage[latin1]{inputenc}

\usepackage{afterpage}

\usepackage{multind}             %multiple Inidices



\usepackage{chicago_new}




\usepackage{amsfonts, amsmath, amssymb, amsthm}
\usepackage{calc}
\usepackage{curves,epic,eepic,latexsym,ifthen}
%new
\usepackage{curves,epic,eepic,amsmath,latexsym,amssymb,array,ifthen,dcolumn}
\usepackage{epsfig}

%new
\usepackage{graphicx}
\usepackage[only,tenrm,svtnrm,egtrm,frtnrm]{rawfonts}

%\usepackage{showkeys}   %Label-Name at margin

\usepackage{rotating}
\usepackage{bbm}

\usepackage{color}
\usepackage{verbatim}
\usepackage{float}
\usepackage{textcomp}
\usepackage[english]{varioref}
\usepackage[scanall]{psfrag}

%Schauberger
\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage{pgfkeys}

\listfiles

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{%
  longtable,
  array,
  booktabs,
  dcolumn,
  rotating,
  shortvrb,
  tabularx,
  units,
  multirow
}

%\usepackage{fltpoint}
%\usepackage{rccol}
%\rcDecimalSign{.}


%% booktabs
\setlength{\heavyrulewidth}{0.06em}    % for \toprule and \bottomrule (default 0.08em)
\setlength{\lightrulewidth}{0.04em}    % for \midrulelightrulewidth (default 0.05em)
    % cmidrulewidht = 0.03em (fr \cmidrule)


%% Tables specific letter type
\newenvironment{tabularsmall}
{
\footnotesize \sffamily
\tabular
}
{
\endtabular
\normalfont
}

%% Ausrichtung am Dezimalpunkt
\newcolumntype{d}[1]{D{.}{.}{#1}} %% d{Anz.Dezimalstellen}


\newcolumntype{.}[1]{D{.}{.}{#1}}  %% in count


%% zum leichteren Ausrichten von Tabellenspalten
\newcommand{\ph}[1]{\phantom{#1}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Pages, Margins
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[
DIVcalc,       % Textbereich (in log-Datei nachlesen)
%DIVclassic
%,headinclude    % dann ist Kopfzeile+Text 18,9cm hoch,
%,headexclude    % dann ist nur der Text 18.9cm hoch + Kopfzeile
%,footexclude    % footinclude
,1.0headlines   %default ist 1.25headlines
%,pagesize
]{typearea}

%\typearea{8}

%\areaset{11.7cm}{18.9cm}
\areaset{13.3cm}{21.0cm}
%kleinerer Abstand von Kopfzeile zu Text
%\setlength{\headheight}{0pt} %13.6pt    holt den Text etwas nï¿½er



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         fancy head and bottom
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fancyhdr}

\pagestyle{fancy}
\lhead[\fancyplain{}{\textrm\thepage}]                            % even page
      {\fancyplain{}{\normalfont\footnotesize\scshape\rightmark}} % uneven page
\rhead[\fancyplain{}{\normalfont\footnotesize\scshape\leftmark}]
      {\fancyplain{}{\textrm\thepage}}
\chead{}

\renewcommand{\headrulewidth}{0.5pt} % Trennlinie
\setlength{\headsep}{10pt}           % kleinerer Abstand Text-Kopfzeile (default ist 25pt)

\lfoot{}
\cfoot{\fancyplain{\textrm\thepage}{}}
\rfoot{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  minipages with boxes
% use  \boxnew[Breite]{Inhalt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\boxtitle}[1]{\begin{center} \sffamily #1 \end{center}}
\newcommand{\boxitem}[1]{\textsf{\small #1}}

\newcommand{\boxnew}[2][0.8\textwidth]{               %0.8\textwidth als default
   \vspace{1.5ex}          %1ex bewirkt nichts, entspricht 100%
   \begin{center}
   \fbox{%
     \begin{minipage}{#1}   %\linewidth-4ex  ergibt textbreiten Kasten
       {#2}%
     \end{minipage}}%
   \end{center}
   \vspace{2ex}
}

\newcommand{\boxcaption}[1]{
\captionsetup{aboveskip=-1.6ex, belowskip=2ex}
\captionof{table}{#1}
\captionsetup{aboveskip=10pt, belowskip=0pt}
\vspace{1.5ex}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Index (neu 6.7.06 von J.Brandt)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sindex}[1]{\index{subjectindex}{#1}}
\newcommand{\aindex}[1]{\index{authorindex}{#1}}

% Zweispaltiger Index
\makeatletter
\renewcommand{\printindex}[2]{
   \@restonecoltrue\if@twocolumn\@restonecolfalse\fi
   \columnseprule \z@ \columnsep 35pt   %%obsolet, besser \setlength
   \newpage
   \@mkboth{\MakeUppercase{#2}}{\MakeUppercase{#2}}      %Fr Kopfzeile
%    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]      %%obsolet, wegen \rm
    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]
   \addcontentsline{toc}{chapter}{#2}                    %Eintrag ins Inhaltsverzeichnis
   \@input{#1.ind}
 }
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Examples including counter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\ecaption}[1]{\addcontentsline{loe}{example}{\protect\numberline{\theexample}#1}} %loe: listOfExamples
\newcommand{\l@example}{\@dottedtocline{1}{0em}{3.2em}}

\newcommand{\listofexamples}{
     \chapter*{List of Examples}                  %ï¿½berschrift der Beispielsliste
     \@mkboth{List of Examples}{List of Examples}         %header
%   \addcontentsline{toc}{section}{List of Examples}    %hier liegt das Problem mit den minitocs => statt chapter nun section und es funktioniert
\addcontentsline{toc}{chapter}{List of Examples}
%     \thispagestyle{empty}
     { \@starttoc{loe}}
}
\makeatother

\newcounter{example}[chapter]
\renewcommand{\theexample}{\thechapter.\arabic{example}}

\newenvironment{example}[1]
    {\refstepcounter{example}
     \ecaption{#1}
     \bigskip
     \noindent{\small \sffamily Example \theexample: #1}
     %\noindent{\small \scshape Example \normalfont \theexample: #1}
                    % Schrift der Beispielsberschrift
     \small         % Schrift des Textes (ohne ï¿½berschrift)
     \\}
    {\qed \bigskip}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Chapter headings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
%% aus book.cls kopiert und modifiziert
\renewcommand\chapter{\if@openright\cleardoublepage\else\clearpage\fi
                    \thispagestyle{plain}%
                    \global\@topnum\z@
                    \@afterindentfalse
                    \secdef\@chapter\@schapter}
\def\@chapter[#1]#2{\ifnum \c@secnumdepth >\m@ne
                       \if@mainmatter
                         \refstepcounter{chapter}%
                         \typeout{\@chapapp\space\thechapter.}%
                         \addcontentsline{toc}{chapter}%
                                   {\protect\numberline{\thechapter}#1}%
                       \else
                         \addcontentsline{toc}{chapter}{#1}%
                       \fi
                    \else
                      \addcontentsline{toc}{chapter}{#1}%
                    \fi
                    \chaptermark{#1}%
                    \addtocontents{lof}{\protect\addvspace{10\p@}}%
                    \addtocontents{lot}{\protect\addvspace{10\p@}}%
                    \if@twocolumn
                      \@topnewpage[\@makechapterhead{#2}]%
                    \else
                      \@makechapterhead{#2}%
                      \@afterheading
                    \fi}
\def\@makechapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright \sffamily  %\normalfont default, jetzt \sffamily
    \ifnum \c@secnumdepth >\m@ne
      \if@mainmatter
        \huge \@chapapp\space \thechapter %\bfseries  %nur fï¿½r das Wort Chapter
        \par\nobreak
        \vskip 20\p@        %20
      \fi
    \fi
    \interlinepenalty\@M
%    \Huge  #1\par\nobreak  %\bfseries       %fï¿½r die eigentliche ï¿½berschrift
    \huge  #1\par\nobreak  %\bfseries
    \vskip 40\p@        %40
  }}
\def\@schapter#1{\if@twocolumn
                   \@topnewpage[\@makeschapterhead{#1}]%
                 \else
                   \@makeschapterhead{#1}%
                   \@afterheading
                 \fi}
\def\@makeschapterhead#1{           %verï¿½ndert die Schrift der ï¿½berschrift des Inhalts-, Beispiels- und Literaturverzeichnisses
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright
    \sffamily                       %\normalfont alt
    \interlinepenalty\@M
%    \Huge   #1\par\nobreak          %\bfseries
    \huge   #1\par\nobreak
    \vskip 40\p@
  }}
%%

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}% Abstand drï¿½ber
                                   {1.1ex \@plus.1ex}      % Abstand drunter
                                   {\sffamily\Large}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.0ex \@plus .1ex}%
                                     {\sffamily\large}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex \@plus .1ex}%
                                     {\sffamily\normalsize}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                    {3.25ex \@plus1ex \@minus.2ex}%
                                    {1ex}%
                                    {\sffamily\normalsize}}
\makeatother

%default-Werte
% \newcommand\section{\@startsection {section}{1}{\z@}%
%                                    {-3.5ex \@plus -1ex \@minus -.2ex}%
%                                    {2.3ex \@plus.2ex}%
%                                    {\normalfont\Large\bfseries}}
% \newcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\large\bfseries}}
% \newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\normalsize\bfseries}}
% \newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
%                                     {3.25ex \@plus1ex \@minus.2ex}%
%                                     {-1em}%
%                                     {\normalfont\normalsize\bfseries}}
% \newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
%                                        {3.25ex \@plus1ex \@minus .2ex}%
%                                        {-1em}%
%                                       {\normalfont\normalsize\bfseries}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Im Anhang bekommen chapter, section und subsection wieder andere Bedeutung
% (noch nicht berarbeitet)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \makeatletter
%   \renewcommand*\l@chapter[2]{%
%     \ifnum \c@tocdepth >\m@ne
%       \addpenalty{-\@highpenalty}%
%       \vskip 1.0em \@plus\p@
%       \setlength\@tempdima{1.5em}%
%       \begingroup
%         \parindent \z@ \rightskip \@pnumwidth
%         \parfillskip -\@pnumwidth
%         \leavevmode \bfseries %\mdseries %\sffamily
%         \advance\leftskip\@tempdima
%         \hskip -\leftskip
%         #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
%         \penalty\@highpenalty
%       \endgroup
%     \fi}
% \renewcommand{\appendixname}{Appendix}
% \renewcommand{\appendix}{%
%   \setcounter{chapter}{0}
%   \renewcommand{\thechapter}{\Alph{chapter}}%
%   \renewcommand{\chapter}[1]{%
%     \cleardoublepage\thispagestyle{plain}%
%     \refstepcounter{chapter}%
%     \addcontentsline{toc}{chapter}%
%       {%\protect\sffamily%
%        \protect\numberline{\protect\bfseries\protect%   %%dazw.\bfseries
%        \protect\appendixname\protect\hspace{1ex}\thechapter:}\protect\hspace{9ex}\protect##1}%
%     \@mkboth{\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%             {\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%     {\flushleft\LARGE\mdseries\sffamily%
%      \appendixname\ \thechapter:\ \nohyphens##1\par}%
%   %\chaptermark{##1}\vspace{\baselineskip}
%   }
%   \renewcommand{\section}[1]{
%     \refstepcounter{section}%
%     \addcontentsline{toc}{section}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesection}##1}%
%     {\noindent\large\mdseries\sffamily\thesection~##1\par}
% %    {\flushleft\large\mdseries\sffamily\thesection~##1\par} ohne Trennungen
%   }
%   \renewcommand{\subsection}[1]{
%     \refstepcounter{subsection}%
%     \addcontentsline{toc}{subsection}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesubsection}##1}%
%     {\noindent\normalsize\mdseries\sffamily\thesubsection~##1\par}
% %    {\flushleft\normalsize\mdseries\sffamily\thesubsection~##1\par} ohne Trennungen
%   }
% }
%% \makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Captions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{caption}[2003/12/20]
\captionsetup{width=\linewidth-2cm,font=footnotesize,labelfont={sc}}
    %font: Einstellung fï¿½r die gesamte Unterschrift
    %labelfont: Einstellung fï¿½r den Bezeichner (``Table'')


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Literature  - neu 1.9.2011 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% aus book.cls %%

\makeatletter

\renewenvironment{thebibliography}[1]
     {\chapter*{\bibname}%
      \@mkboth{\MakeUppercase\bibname}{\MakeUppercase\bibname}%
      %     {\rm\Large\sffamily\mdseries \bibname\vskip2ex}     %ergänzt
    \addcontentsline{toc}{chapter}{\bibname}    %ergänzt
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}

\makeatother

\let\oldbibliography\thebibliography
\renewcommand{\thebibliography}[1]{%
\oldbibliography{#1}%
%\setlength{\itemsep}{0ex}           %% Abstand zwischen den Einträgen %%
\setlength{\itemsep}{-0.3ex} }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         minitocs: kleine Inhaltsverzeichnisse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{minitoc}       % kleine Inhaltsverzeichnisse
\setlength{\fboxsep}{1em}  % \fboxsep4mm    %Vergleiche Einstellungen fï¿½r \boxnew
\setlength{\mtcindent}{4pt}
\renewcommand{\mtcfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSSfont}{\small\mdseries\sffamily}

\newcommand{\makeminitoc}{%
\setcounter{minitocdepth}{3}    % Anzahl Gliederungsebenen
   \vspace{3mm}
   \hrule
   \bigskip
   \noindent


%   \fbox{%
   \begin{minipage}{\linewidth -5ex}
     \vspace*{-3ex}
     \nomtcrule
     \minitoc
\hrule
\bigskip
%     \vspace*{-5ex}%3
   \end{minipage}
%   }
\\[3mm]}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Applications   ** neu 21.10.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Applications innerhalb der Umgebung
\newcounter{application}[chapter]
\renewcommand{\theapplication}{\thechapter.\arabic{application}}

%% Definition der Umgebung 'application'
\newenvironment{application}
    {\refstepcounter{application}
     \bigskip
     \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
     \\
     \small         % Schrift des Textes (ohne Ueberschrift)
     }

    { \bigskip}

%% Fuer leichtere (a), (b), (c) AufzÃ¤hlungen
\usepackage{enumitem}

\newenvironment{abcitemize}
    {\begin{enumerate}[label=(\alph*)]}
    {\end{enumerate}}


% \newenvironment{anwendung}[1]
%     {\refstepcounter{application}
%      \bigskip
%      \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
%      \small         % Schrift des Textes (ohne Ueberschrift)
%      \\
%      #1
%      \begin{enumerate}[label=(\alph*)]
%      }
%     { \end{enumerate} \bigskip}







% %% Variante 2 *****************************************************************

%
%
% \renewcommand{\labelenumi}{\small \textsf{Application \theenumi :}}
%
%
% \newenvironment{anwendungen}%[Ã]
% {\small \begin{enumerate}[leftmargin=*, style=nextline] }
% {\end{enumerate} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Exercises   ** neu 19.11.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Exercieses
\newcounter{exercise}[chapter]
\renewcommand{\theexercise}{\thechapter.\arabic{exercise}}

%% Definition der Umgebung 'exercise'
\newenvironment{exercise}
    {\refstepcounter{exercise}
     \bigskip \small
     \noindent \theexercise
     }

    { \bigskip}

